A Nearly Quadratic Improvement for Memory Reallocation

In the Memory Reallocation Problem a set of items of various sizes must be dynamically assigned to non-overlapping contiguous chunks of memory. It is guaranteed that the sum of the sizes of all items present at any time is at most a $(1-\varepsilon)$-fraction of the total size of memory (i.e., the load-factor is at most $1-\varepsilon$). The allocator receives insert and delete requests online, and can re-arrange existing items to handle the requests, but at a reallocation cost defined to be the sum of the sizes of items moved divided by the size of the item being inserted/deleted. The folklore algorithm for Memory Reallocation achieves a cost of $O(\varepsilon^{-1})$ per update. In recent work at FOCS'23, Kuszmaul showed that, in the special case where each item is promised to be smaller than an $\varepsilon^4$-fraction of memory, it is possible to achieve expected update cost $O(\log\varepsilon^{-1})$. Kuszmaul conjectures, however, that for larger items the folklore algorithm is optimal. In this work we disprove Kuszmaul's conjecture, giving an allocator that achieves expected update cost $O(\varepsilon^{-1/2} \operatorname*{polylog} \varepsilon^{-1})$ on any input sequence. We also give the first non-trivial lower bound for the Memory Reallocation Problem: we demonstrate an input sequence on which any resizable allocator (even offline) must incur amortized update cost at least $\Omega(\log\varepsilon^{-1})$. Finally, we analyze the Memory Reallocation Problem on a stochastic sequence of inserts and deletes, with random sizes in $[\delta, 2 \delta]$ for some $\delta$. We show that, in this simplified setting, it is possible to achieve $O(\log\varepsilon^{-1})$ expected update cost, even in the ``large item'' parameter regime ($\delta > \varepsilon^4$).

==> extra_small_items.tex <==
%%%%%%%%%%%%%%%%%%SECTION: SMALL ITEMS%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{An $\bigO(1)$-cost allocator for small items}\label{sec:small}
Kuszmaul's \tinyhash allocator already is capable of handling items of size at most $\eps^4$ at cost $\bigO(\log \eps^{-1})$.
There is a known construction to handle the case where 
all items have size between  $(\eps^{3}, 2\eps^3)$  with  $\bigO(1)$ update cost.
In this section we show that this construction can be extended 
to achieve $\bigO(1)$ cost on larger items, e.g., items with sizes in the range $(\eps^{2.1}, 2\eps^{100})$.
We also show how to combine these ideas with Kuszmaul's \tinyhash 
to obtain an allocator that
handles any items of size at most $\eps^{2}/\log \eps^{-1}$ 
at update cost $\bigO(\log \eps^{-1})$.

This section is significant because it further narrows the 
parameter regime where we only have $\poly(\eps^{-1})$ update cost algorithms.

\begin{theorem}\label{thm:smallitems}
Fix $\gamma\in (0,1/4)$ with $\gamma^{-1} \le
\bigO(\sqrt{\log\eps^{-1}})$.
Assume all items have size between $(\eps^{2+\gamma}, \eps^{5})$.
There is an allocator for such items with amortized update cost $\bigO(\gamma^{-1})$.
\end{theorem}
\begin{proof}
  We call our allocator \block. \block geometrically discretizes
  the items into $C\le \bigO(\eps^{-1}\log(\eps^{-1}))$ sizes by
  rounding item sizes up to the next largest multiple of
  $(1+\eps)^{-i}$. Fix integer $\ell>1$ such that $ \gamma / 4 < \frac{1}{\ell-1} < \gamma/2$.
  Let $a = 2+\gamma$.

  \block maintains $\ell$ \defn{mem-blocks} of sizes
  $M_1,M_2,\ldots, M_{\ell}$. \block chooses the mem-block sizes so
  that for each $i\in [\ell]$ 
  $$M_i \in \Theta\left( \eps^{\frac{\ell-i+ia}{\ell+1}} \right),$$ 
  and also so that for each $i\in [\ell-1]$ there is some integer
  $k$ such that $M_i/M_{i+1} = k$. Furthermore we choose $M_1$ so
  that there is some $k$ for which $1/M_1 = k$.
  For each item size \block maintains an \defn{active} mem-block,
  which will be of size $M_{\ell}$.
  \block will maintain the following invariants:
  \begin{itemize}
      \item Each mem-block is restricted to containing a
        single size of element. An $x$-mem-block will denote a
        mem-block that is only allowed to hold items of size
        $x$. 
      \item For each item size $x$ and each $i\in [\ell-1]$ there
        are never more than $(3/2) M_{i}/M_{i+1}$ $x$-mem-blocks
        of size $M_{i+1}$.
      \item For each $i\in [\ell]$ mem-blocks of size $M_i$ must start at a location
        $jM_i$ for some integer $j\ge 0$.
  \end{itemize}

  Now we describe how \block handles updates.
  We give pseudocode in \cref{alg:small-blocks}, with subroutines
  described in \cref{alg:fracture}, \cref{alg:place}, and \cref{alg:merge}.

    \begin{algorithm}
      \caption{Fracture}\label{alg:fracture}
        \begin{algorithmic}[1]
          \Procedure{fracture}{item size $x$}
          \State Let $i\in [\ell]$ be the largest $i$ such that there is an $x$-mem-block of size $M_i$.
          \State \textbf{Assert:} $i<\ell$. \label{assert:not_fracture_l}
          \State Select an $x$-mem-block $B$ of size $M_i$.
          \State Destroy $B$, and redistribute its elements into smaller mem-blocks as follows:
          \State Make a mem-block of size $M_\ell$. Then, for each $i'>i$ make as many mem-blocks of size $i'$ as possible.
          \State \textbf{Assert:} the previous  step creates
          fewer than $(3/2)M_{i-1}/M_{i}$ memory blocks of size
          $M_i$ for all $i$.
          \label{assert:fracture-not-violate-invar}
          \State Let $\mathcal{B}$ be the set of newly created mem-blocks. 
          \State For each mem-block $B' \in \mathcal{B}$, $\place(B')$
          \EndProcedure
        \end{algorithmic}
    \end{algorithm}

    \begin{algorithm}
      \caption{Place}\label{alg:place}
        \begin{algorithmic}[1]
          \Procedure{Place}{mem-block $B$}
          \State Let $M_i$ denote the size of mem-block $B$.
          \State Find a memory region $(jM_i, (j+1)M_i)$ for
          $j\in \Z_{\ge 0}$ which is not occupied by any mem-blocks of size at least $M_i$.
          \State \textbf{Assert:} the command on the previous
          line is possible, i.e., some such region exists.
          \label{assert:can-find-place}
          \State Let $\mathcal{B}$ be the set of mem-blocks already present in
          the found memory region.
          \State Put mem-block $B$ in location $(jM_i, (j+1)M_i)$, displacing mem-blocks $\mathcal{B}$.
          \State For each displaced mem-block $B'\in \mathcal{B}$, $\place(B')$.
          \EndProcedure
        \end{algorithmic}
    \end{algorithm}

    \begin{algorithm}
      \caption{Merge}\label{alg:merge}
        \begin{algorithmic}[1]
          \Procedure{Merge}{$x, M_i$}
          \State \textbf{Assert:} $i\neq 1$.
          \State \textbf{Assert:} if $i\neq 2$ then there are fewer than
          $(5/4)M_{i-2}/M_{i-1}$ $x$-mem-blocks of size
          $M_{i-1}$.\label{assert:merge-next-small}
          \label{assert:dont-merge-1}
          \While{there are more than $(5/4)M_{i-1}/M_{i}$ $x$-mem-blocks of size $M_i$}
              \State Let $m = \floor{M_{i-1}/x}$ be the maximum
              number of size $x$ items that fit in a
              $M_{i-1}$-sized mem-block.
              \State Let $k$ be the minimum number of $M_{i}$-sized
               $x$-mem-blocks so that in total there are at least
               $m$ items amongst these $m$ mem-blocks.
               \State Destroy $k$ $M_i$-sized $x$-mem-blocks, and
               let $S$ be the set of items that were in these mem-blocks.
               \State In the above step, the active mem-block is
               not allowed to be one of the destroyed mem-blocks.
            \State Re-organize the items $S$ into mem-blocks as follows:
          \State Make a mem-block of size $M_{i-1}$. Then, for
          each $i'>i$ make as many mem-blocks of size $i'$ as
          possible.
          \State Let $\mathcal{B}$ be the set of newly created mem-blocks. 
          \State For each mem-block $B' \in \mathcal{B}$, $\place(B')$
          \EndWhile
          \State \textbf{Assert:} If $i\neq 2$ there are fewer than
          $(3/2)M_{i-2}/M_{i-1}$ $x$-mem-blocks
          $x$-mem-blocks of size
          $M_{i-1}$.\label{assert:merge-no-upwards-stream}
          \State \textbf{Assert:} There are fewer than
          $(5/4)M_{i-1}/M_i$  $x$-mem-blocks of size
          $M_i$.\label{assert:merge-lol-we-merged}
          \EndProcedure
        \end{algorithmic}
    \end{algorithm}

    \begin{algorithm}
        \caption{\block Allocator}\label{alg:small-blocks}
        \begin{algorithmic}[1]
          \If{an item $I$ of size $x$ is deleted}
            \If{size-$x$'s active mem-block becomes empty, and
            there is some other $x$-mem-block}
              \State Free size-$x$'s active mem-block, i.e., no
              longer consider it an $x$-mem-block.
              \If{there are no other $x$-mem-blocks of size $M_\ell$}
              \State  $\fracture(x)$.
              \EndIf
            \EndIf
              \State \textbf{Assert:} now there is an $x$-mem-block of size $M_\ell$.
              \label{assert:block-fracture-succeeds}
              \State Arbitrarily designate an $x$-mem-block
              of size $M_\ell$ as size-$x$'s  active mem-block.
          \ElsIf{an item $I$ of size $x$ is inserted}
          \If{there is insufficient room for $I$ in size-$x$'s active mem-block}
              \State \textbf{Assert:} there is an empty memory
              region $(jM_\ell, (j+1)M_\ell)$ for some $j\in
              \Z_{\ge 0}$.
              \label{assert:empty-region-exists}
            \State Find $j\in \Z_{\ge 0}$ so that memory $(jM_\ell,
            (j+1)M_\ell)$ is empty and designate it as an $x$-mem-block. 
            \State Set this empty $x$-mem-block to be size-$x$'s active mem-block.
            \If{the number of $x$-mem-blocks of size $M_\ell$ exceeds $(3/2) M_{\ell-1}/M_\ell$}
            \State Let $i_0$ be the smallest
            $i\in[\ell]\setminus [1]$ so that there are at least $(5/4)M_{i-1}/M_i$ size-$M_i$ $x$-mem-blocks.
            \For{$i \gets i_0, i_0+1, \ldots, \ell$}
                \State $\merge(x,M_i)$.
            \EndFor
            \EndIf
            \State \textbf{Assert:} there are at most $(3/2) M_{i-1}/M_{i}$ $x$-mem-blocks of size $M_i$ for each $i\in [\ell]\setminus [1]$.
            \label{assert:merge-hou-invar-holds}
          \EndIf
          \State \textbf{Assert:} size-$x$'s active mem-block has sufficient space for item $I$.
          \label{assert:can-fit}
            \State Place $I$ in size $x$'s active mem-block.
          \EndIf
        \end{algorithmic}
    \end{algorithm}

    \begin{figure}
        \centering
        \includegraphics[width=\linewidth]{images/small-items.pdf}
        \caption{small-items}
        \label{fig:small-items}
    \end{figure}

Now we explain the pseudo-code in more detail.
At a high level the allocator works as follows:
\begin{itemize}
    \item  Whenever an item of size $x$ is inserted it is 
placed into the active mem-block for size $x$.
\item  Whenever an item of size $x$ is deleted we 
replace it with an item from the active mem-block for size $x$. 
\end{itemize}
We encounter difficulties in two cases: 
(1) when we delete the final item of an active mem-block,
(2) when there is no more room in the active mem-block for more items.

We handle (1) as follows:
When the final item of size $x$ is deleted we allow size $x$ to have an empty active mem-block.
If the deleted item is not the last of its size there must be some other $x$-mem-block. 
If there is another $x$-mem-block of size $M_\ell$ 
we can simply designate this as the new active mem-block for size
$x$, \defn{freeing} the old active mem-block. If there are only
larger $x$-mem-blocks then we must perform a \defn{fracture}
operation, in which we split up a larger $x$-mem-block to create
smaller $x$-mem-blocks, and in particular one of size $M_\ell$ to
become the new active mem-block for size $x$.

A fracture operation works as follows:
Choose an $x$-mem-block of the smallest size 
and destroy it, redistributing its elements into smaller mem-blocks.
In particular, make sure to create a $M_\ell$-sized mem-block, 
and then prioritize creating the biggest possible mem-blocks.
To complete the fracture operation we then must 
perform a \defn{place} operation on each of the newly created mem-blocks.

A place operation works as follows:
Find an appropriate location to put the mem-block
that is not occupied by any mem-blocks of the same size or larger.
Place the mem-block in this location and then recursively 
place any displaced smaller mem-blocks.

Now we describe how to handle (2), i.e., what to do 
on an insert when there is no room left in the active mem-block.
In this case, \block creates a new active mem-block 
and puts the item in this new active mem-block.

This may result in \block's invariant on the maximum 
allowed number of $M_\ell$-sized $x$-mem-blocks being violated.
In this case \block must perform a \defn{merge} operation to restore the invariant.

A merge operation works as follows:
\block computes $i_0$ which is the 
smallest $i\in [\ell]\setminus [1]$ such that 
there are a lot of blocks of size $M_i$, 
specifically more than $(5/4)M_{i-1}/M_i$.
Then, for $i\gets i_0, i_0+1, \ldots, \ell$ \block does the following:
\block combines $M_i$-sized mem-blocks to form a $M_{i-1}$ mem-block, 
and forms some smaller mem-blocks with any left-over items.
\block then performs place operations on all newly created mem-blocks.

Now we argue for the algorithms correctness. 
\begin{lemma}\label{lem:block-correct}
    \block is well-defined, i.e., it maintains the promised invariants and 
    the assert statements in the pseudocode are never triggered.
\end{lemma}
\begin{proof}
The invariant that $x$-mem-blocks only ever store items of size
$x$ is clearly satisfied by construction.
The invariant that $M_i$-sized mem-blocks start at positions
$jM_i$ for some  $j\in \Z_{\ge 0}$ holds because whenever we
create a new mem-block or do a place operation  to move a
mem-block we make sure to put  the mem-block at a correctly
aligned position.
The invariant that there are never more than $(3/2)M_{i-1}/M_i$
mem-blocks of size $M_i$ is guaranteed by the assert statement in
the fracture code and the assert statement after merge is called.

Now we analyze what the gaps in the array that \block allows look like. 
Let the \defn{total-block-size} denote the sum of the sizes of
all of \block's blocks, and let the \defn{total-present-size} be
the sum of the sizes of all present items.
We claim:
\begin{claim}\label{clm:waste-no-more}
  The total-block-size is at most $\eps$ more than the
    total-present-size.
\end{claim}
\begin{proof}
  \block has an active block, of size $M_\ell$, for each of the
  $C$ item sizes which is allowed to be empty. This contributes
  $C M_\ell$ to the wasted space. 
  All non-active blocks are essentially completely full, modulo a
  tiny gap at the end due to the fact that item sizes don't
  perfectly divide into the sizes $M_i$.
  For each  $i\in [\ell]\setminus[1]$ the wasted space on
  $M_i$-sized mem-blocks  is at most:
  $$\frac{3}{2} \frac{M_{i-1}}{M_{i}}\cdot \eps^a  \cdot C.$$
  Finally, there are at most $1/M_1$ mem-blocks of size $M_1$,
  and so the wasted space due to the gaps in these size of
  mem-blocks is at most 
$$\frac{1}{M_1}\eps^a.$$

Adding up these contributions, we find the waste to be at most 
\begin{equation}\label{eq:all-waste-small}
\frac{\eps^{a}}{M_1} + \frac{3}{2}\frac{M_{i-1}}{M_i}\eps^{a}C + CM_\ell.
\end{equation}
We bound the first term of \cref{eq:all-waste-small} as 
$$\eps^{a}/M_1 = \eps^{a - \frac{\ell-1+a}{\ell+1}} =
\eps^{1+\gamma - \frac{\gamma}{\ell+2}} \le \eps^{1+\gamma/2}.$$
We bound the second term of \cref{eq:all-waste-small} as 
$$\frac{3}{2}\frac{M_{i-1}}{M_i}\eps^{a}C \le
\eps^{\frac{1-a}{\ell+1}}\eps^{a}\eps^{-1}\bigO(\log\eps^{-1})
\le \eps^{1+\gamma-\frac{1+\gamma}{\ell+1}}\bigO(\log\eps^{-1}).$$

Using the fact that we chose $\ell-1> 2/\gamma$ we derive
$\ell+1> \frac{1+\gamma}{\gamma/2}$, and then 
$\gamma - \frac{1+\gamma}{\ell+1}>\gamma/2$ so
$$1+\gamma - \frac{1+\gamma}{\ell+1} > \gamma/2.$$
Thus, the second term of \cref{eq:all-waste-small} is bounded by:
$$\bigO(\log\eps^{-1})\eps^{1+\gamma/2}.$$
Finally we bound the third term of \cref{eq:all-waste-small} as 
$$CM_\ell \le \bigO(\log\eps^{-1})
\eps^{\frac{\ell+\gamma\ell-1}{\ell+1}}.$$
Using the fact that we chose $\ell-1<4/\gamma$ we derive
$$\frac{\ell+\gamma\ell-1}{\ell+1}<1+\gamma/2.$$
Thus, the third term of \cref{eq:all-waste-small} is bounded by 
$$\bigO(\log\eps^{-1})\eps^{1+\gamma/2}.$$

Adding up all the quantities the wasted space is bounded by 
$$\eps^{2+\gamma/2} (\log\eps^{-1})^2 \le \eps$$
because we restricted to $\gamma\le \bigO(\sqrt{\log\eps^{-1}})$,
and because our analysis is asymptotic (i.e., we assume $\eps$ is
sufficiently large so that the inequality holds).
\end{proof}

Finally, we argue that the assert statements in our pseudocode
are always true.
\begin{itemize}
  \item \cref{assert:not_fracture_l} holds because we only call
    fracture if there are no other $M_\ell$-sized
    $x$-mem-blocks.
  \item To verify \cref{assert:fracture-not-violate-invar}
    it suffices to show that when a $M_i$-sized mem-block splits
    it creates at most $(4/3)M_{j-1}/M_j$ mem-blocks of size
    $M_j$ for all $j>i$.
    The total mass of items amongst $(4/3)M_{j-1}/M_j$
    mem-blocks of size  $M_j$ is at least
    $$(4/3) \frac{M_{j-1}}{M_j} (M_j - \eps^{a}) \ge M_{j-1},$$
   due to the fact that 
   $$M_\ell = \Theta(\eps^{\frac{a\ell}{\ell+1}}) \ge 4\eps^{a}.$$
 \item Imagine that \cref{assert:can-find-place} fails. This
   would imply, due to the alignment invariant, that the
   total-block-size is $1$. Then, by \cref{clm:waste-no-more} we
   have that the total-present-size is $1-\eps$. But, this means
   that after the new item is inserted the total-present-size
   would exceed $1-\eps$. This is impossible, because we are
   guaranteed that the total-present-size never exceeds $1-\eps$. 
 \item \cref{assert:dont-merge-1} is trivially true: we never try
   to merge mem-blocks of size $M_1$. This is ok, because we
   don't have a strict constraint on the maximum number of
   $M_1$-sized $x$-mem-blocks, as opposed to for $M_i$ for $i>1$.
 \item \cref{assert:block-fracture-succeeds} is true because
   the fracture procedure prioritizes creating a mem-block of
   size $M_\ell$.
 \item Imagine that \cref{assert:empty-region-exists} fails.
  This would imply, due to the alignment invariant, that the
   total-block-size is $1$. Then, by \cref{clm:waste-no-more} we
   have that the total-present-size is $1-\eps$. But, this means
   that after the new item is inserted the total-present-size
   would exceed $1-\eps$. This is impossible, because we are
   guaranteed that the total-present-size never exceeds $1-\eps$.
 \item \cref{assert:merge-hou-invar-holds} is ensured by 
   the assertions \cref{assert:merge-no-upwards-stream} and
   \cref{assert:merge-lol-we-merged}. In
   particular, at each step of the for-loop we ensure that there
   are at most $(5/4)M_{i-1}/M_i$  $x$-mem-blocks of size $M_i$.
   So by the end we will have restored the invariant for
   $M_\ell$, which is where it was initially broken.
 \item \cref{assert:can-fit} is true because either the
   if-conditional checking if there was enough space is
   triggered, in which case we create a new empty mem-block, or
   the if-conditional was not triggered, in which case the room
   was already sufficient.
 \item \cref{assert:merge-next-small} is true on the first
   iteration of the for-loop where we call merge because we
   choose the first $i$ where we call the merge operation to
   satisfy the condition. On subsequent steps of the for-loop the
   guarantee is satisfied by virtue of
   \cref{assert:merge-lol-we-merged} for the call of merge in the
   previous iteration of the for-loop.
 \item \cref{assert:merge-no-upwards-stream} is true because of
   \cref{assert:merge-next-small} and because the total number of
   mem-blocks of size $M_{i-1}$ that you could possibly create by
   combining all items in mem-blocks of size at most $M_i$ is at
   most $2$.\todo{urgh this is technically not quite true?
   because fractures are freaking weird.}
 \item \cref{assert:merge-lol-we-merged} is true because we
   continue in the while loop destroying $x$-mem-blocks of size
   $M_i$ until there are fewer than $(5/4)M_{i-1}/M_i$
   $x$-mem-blocks of size $M_i$.
\end{itemize}

\end{proof}

Now we analyze the performance of the allocator:
\begin{lem}
  The allocator incurs amortized update cost $\bigO(\gamma^{-1})$.
\end{lem}
\begin{proof}
\todo{pretty much the only concerning thing is fracture / merge
steps and this is what their amortized work should look like.}
\end{proof}
    
\end{proof}

% \todo{an interesting question: can you somehow get 
% $\bigO(1)$ for arbitrarily small items with a geometric approach?}

\begin{corollary}
  Assume all items have size at most $\eps^{2}\cdot
  \bigO(2^{\sqrt{\log \eps^{-1}}})$.
There is an allocator for such items with amortized update cost $\bigO(\log(\eps^{-1}))$.
\end{corollary}
\begin{proof}[Proof sketch]
  We use \block with $\gamma\in \Theta(1/\sqrt{\log \eps^{-1}})$ together with
Kuszmaul's allocator. Unfortunately the \block allocator of
\cref{thm:smallitems} is not resizable. In fact, it seems
challenging to make it resizable. Fortunately we do not need such
a strong property: the \block allocator already is quite
compatible with Kuszmaul's construction.

In particular, both \block and \tinyhash consist of blocks, which
all nest inside blocks of some maximum sizes
$L_\block<\bigO(\eps^3), L_\tinyhash < \eps^{1+1/\gamma^2}$.

In particular, this means we can combine the two allocators as
follows: they literally just operate on the same pool of memory
and can access memory in $L_{\block}$ chunks.
\todo{formalize}
\end{proof}



==> extra_zt_stuff.tex <==
\begin{prop}
  There is an allocator with average update cost $\bigO\left(
    \frac{t\log n}{\log t}\right)$ in the $t$-item zero-tolerance
    setting.
\end{prop}
\begin{proof}
  We illustrate the idea for $t=n^{1/3}$. The generalization is
  straightforward.
  We call our allocator \fish.
 We have buckets $B_1,B_2$ of maximum sizes $n^{1/3}, n^{2/3}$ and
 fishing-pools $P_1,P_2$ of sizes $n^{2/3}, n$.

 \fish has \defn{big phases} of length $n^{2/3}$ and
 \defn{little phases} of length $n^{1/3}$.
 During a little phase \fish tries to get stuff from the bucket
 $B_1$. But on the power-of-two-numbered requests for any color,
 e.g., on the $64$-th request for a green item, \fish will fault,
 meaning that the bucket $B_1$ ran out of green and \fish needs
 to go fish in  $P_1$ for greens. In particular, if it was the
 $2^{i}$-th request for color X then \fish will take  $2^{i}$ X's
 from $P_1$. $P_1$ will start each little phase being
 \defn{balanced}, i.e., with the same proportion of each item in
 all suffixes of multiple-of-$t$ length. 
 Thus, the fishing will only require looking through a suffix of
 $2^{i+1}t$ items of $P_1$. 
 Also put inserts in bucket $B_1$. Or maybe keep a separate
 insert bucket. It doesn't matter. 

 The little phase will end at some point when the bucket
 $B_1$ overflows. At this point we need to rebuild $P_1$ to make
 it balanced. 
 $B_1$ is allowed to take stuff from bucket $U_2$. If it faults
 in $U_2$ then we dyadically fish $B_2$.

 And then also there are big phases. When $B_2$ overflows we do a
 big phase. At this point we can just rebuild the entire array so
 that's nice. 

 This gives $3n^{1/3}$ vibes. 
 In general it would be $kn^{1/k}$ if $t=n^{1/k}$.

\end{proof}

We remark that this implies that $\Theta(t)$ is the right answer
if $t\in n^{\Omega(1)}$, and that $\Theta(\log n)$ is of course the right
answer if $t\in \bigO(1)$. 
